BiPhone: Modeling Inter Language Phonetic Influences in Text

A large number of people are forced to use the Web in a language they have low literacy in due to technology asymmetries. Written text in the second language (L2) from such users often contains a large number of errors that are influenced by their native language (L1). We propose a method to mine phoneme confusions (sounds in L2 that an L1 speaker is likely to conflate) for pairs of L1 and L2. These confusions are then plugged into a generative model (Bi-Phone) for synthetically producing corrupted L2 text. Through human evaluations, we show that Bi-Phone generates plausible corruptions that differ across L1s and also have widespread coverage on the Web. We also corrupt the popular language understanding benchmark SuperGLUE with our technique (FunGLUE for Phonetically Noised GLUE) and show that SoTA language understating models perform poorly. We also introduce a new phoneme prediction pre-training task which helps byte models to recover performance close to SuperGLUE. Finally, we also release the FunGLUE benchmark to promote further research in phonetically robust language models. To the best of our knowledge, FunGLUE is the first benchmark to introduce L1-L2 interactions in text.

==> do_not_change_related_work_orig.tex <==
\section{Related Work}
% Goal is to show what relevant literature has focus
Summary of a few related papers:
\begin{itemize}
\item \textbf{Cross-lingual and Multilingual Spoken Term Detection for Low-Resource Indian Languages}:

Problem: Looking for a term (or word) provided as text in an audio in a low-resource language -> the problem is called Spoken Term Detection. Overall idea is to use an ASR model trained on another language to obtain the transcript of the audio and look for the term with a slightly relaxed matching criteria. The transcript and keyword are converted to the same phone set and an alignment algorithm is used. They additionally also group similar phonemes together in a phonetic class. (They don’t mention how they do this classification, but I assume it is manual and they have a table in the paper with the classes). 
The phoneme error rate when using an ASR of similar language is lesser than a more diverse language as one would expect. However, the finding is that with the relaxed matching criteria, the spoken term detection is reasonably good even with a dissimilar language ASR. Further incorporating a target-language LM and target language lexicon into the ASR helps increase the chances of finding the exact word or word fragments. (Again, the method of replacing the LM and lexicon in the ASR with the target language LM and lexicon is not very clear. I assume it is to do with understanding/ knowing the ASR model).

\item \textbf{A Unified Phonological Representation of South Asian Languages for Multilingual Text-to-Speech}:

Problem: Text-to-Speech (TTS) needs a lot of resources. The idea is to reduce the amount of training data required while training a new TTS by leveraging existing TTS in other similar languages. In this work they want to experiment pooling the training data from languages with somewhat less overlap in their sound systems. Hence they consider “South Asian languages from 2 different families: Indo-Aryan and Dravidian”. For TTS, the input to their acoustic model is derived from the linguistic transcription and from the metadata. More specifically, in their case, the transcription is a sequence of phonemes in each language. These are converted to IPA (International Phonetic Alphabet) to have uniform representation of the input features for the acoustic model. (The IPA is actually further converted to articulatory vectors using available phonological resources [Funbund: https://aclanthology.org/L18-1353.pdf] ). The novelty of this work is the phonological inventory design.
\end{itemize}

\subsection{Speech - related}: 

\begin{itemize}
\item \textbf{Accent modification for speech recognition of non-native speakers using neural style transfer} - (Feb 2021) https://asmp-eurasipjournals.springeropen.com/articles/10.1186/s13636-021-00199-3 - Motivation: “Accuracy decreases significantly when the ASR system is being used with a non-native speaker of the language to be recognized. The main reason for this is specific pronunciation and accent features related to the mother tongue of that speaker, which influence the pronunciation. At the same time, an extremely limited volume of labeled non-native speech datasets makes it difficult to train, from the ground up, sufficiently accurate ASR systems for non-native speakers.”
Approach: Uses accent style transfer to design a pipeline for modifying the speech of a non-native speaker so that it more closely resembles the native speech
Dataset: English language pronounced by Japanese speakers (UME-ERJ dataset) as well as American speakers. (need to write to authors for dataset)
Downstream task: show that there is a significant relative improvement in terms of the speech recognition accuracy.
Metrics: WER, CER 
A few points: They call out the “lack of labeled datasets of non-native speech which would be large enough to be used as a training set in a supervised learning algorithm.” And hence allude to using an unsupervised approach.
 
\item \textbf{Non-native English speakers' speech correction, based on domain focused document} - https://dl.acm.org/doi/abs/10.1145/3011141.3011169 - (Nov 2016)
Motivation: Speech correction of non-native speakers at international communities such as university students, especially involving discussions about a specific subject/domain. Assumes a domain-focused document
Approach: SR to get initial text, uses HMM method to get the correspondence with the document and extract the sentences. Speech and sentences fed to speech correction module. 
Dataset: A masters thesis
Metrics: WER
 
\item \textbf{Accent Classification in Human Speech Biometrics for Native and Non-native English Speakers}
(June 2019) https://dl.acm.org/doi/10.1145/3316782.3322780
Motivation: “Accent classification provides a biometric path to high resolution speech recognition. This preliminary study explores various methods of human accent recognition through classification of locale.”  “Specifically, non-native English speakers often encounter issues when attempting to converse with automated assistants, and thus measures are required to be able to correctly recognise the accent or locale of a speaker, which can then be logically
acted on accordingly.”
Approach: Classical, ensemble, timeseries and deep learning techniques are all explored and compared
Dataset: spoken sounds from the English phonetic dictionary are grouped based on the locale of the speaker. Speakers are both native (West Midlands, UK; London, UK) and non-native (Mexico City, MX; Chihuahua, MX) English speakers producing a four-class problem. (provided url, but 404: https://www.kaggle.com/birdy654/speech-recognition-dataset-englandand-mexico )
Downstream task: native identification (ensemble performs the best)
Main contributions: (i) A benchmark of the most common model of HMM used for contemporary voice recognition, when training from a uniform spoken audio dataset and producing predictions of speaker accent/locale. (ii) single and ensemble methods for classification (iii) comparison of 11 models
 
\item \textbf{Dual supervised learning for non-native speech recognition (Jan 2019)}
Motivation: “difficult to train or build sufficiently accurate ASR systems targeted at non-native speakers, which, consequently, calls for a different approach that would make use of vast amounts of large unlabeled datasets.”
“Unlabeled data” refers to “speech samples without corresponding transcripts and text corpora without corresponding speech samples”.
Approach: dual supervised learning (DSL) and reinforcement learning with policy gradient methodology. They have 2 pretrained models: one for text LM and the other for Speech. The setup contains 2 more models: a speech recognition model (MSTT), which can recognize phonemes for a given sound sequence. The other one, complementary to the first, is a speech generation model (MTTS), with the functionality of generating a speech signal for a given textual sentence. The latter 2 are part of the DSL. All are in a feedback loop for training (however the pretrained models are not finetuned in this case, and only the STT and TTS models are).
Dataset:  (UME-ERJ) . For training language models ML, they used the Corpus of Contemporary American English (COCA). For training acoustic models MS, we used pieces of recordings scraped from Youtube website resources (mostly either Japanese people teaching Japanese to an English audience, or Japanese expatriates living abroad and creating videos in English). The same source was used in the case of Polish people pronouncing English sentences.
Downstream:  creating ASR systems with DSL can achieve an accuracy comparable to traditional methods, while simultaneously making use of unlabeled data, which obviously is much cheaper to obtain and comes in larger sizes.
Metric: CER
\end{itemize}

\subsection{NLI-related (Native Language Identification)}
\begin{itemize}
\item \textbf{Improving Native Language Identification by Using Spelling Errors}: https://www.aclweb.org/anthology/P17-2086.pdf  (ACL 2017 short paper): 
Data: TOEFL11 corpus (Blanchard et al., 2013) [TOEFL: Test of English as a Foreign Language] Also uses the ICLEv2 corpus (Granger et al., 2009) for extracting additional spelling errors.
Spelling errors as a binary feature: “The errors made by a writer while writing in their L2 may result from sound-to-character mappings in L1, writing preferences or other biases. These could be strong indicators for an author’s L1. We extract spelling errors using the spell shell command.” 
Spelling errors as character n-grams: “Every misspelled word in a text will be represented as character n-grams (n=1..3)”
Other features: word n-grams, lemma n-grams (capture lexical choice of writer), character n-grams (captures information about the preference of an author in using certain sounds, combinations of sounds, prefixes or suffixes.)
Model: SVM classifier to id native language as Hindi, Telugu, Arabic, Spanish, Italian, French, German, Turkish, Chinese and Japanese. 

\item \textbf{Determining an author's native language by mining a text for errors} https://dl.acm.org/doi/10.1145/1081870.1081947   (ACM SIGKDD 2005, an early work on this topic): 
Features include the frequency of function words, rare POS bigrams, letter n-grams, and spelling errors. Classify into 1 of the 5 native European languages using SVMs.

\item \textbf{Cognate and Misspelling Features for Natural Language Identification} (https://www.aclweb.org/anthology/W13-1718.pdf ): 
Misspellings: extract the spelling error features from character-level alignments between the misspelled word and the intended word. The spell-checker we use is aspell (http://aspell.net), and the character-level alignments are generated by m2maligner (Jiampojamarn et al., 2007).
Cognate interferences: “Cognates are words that share their linguistic origin. For example, English become and German bekommen have evolved from the same word in a common ancestor language. Cognate interference may cause an L1-speaker to use a cognate word instead of a correct English translation. We aim to detect cognate interference by identifying the cases where the cognate word is closer to the misspelling than to the intended word.”
Meta features: average number of words per sentence, the average word length, as well as the total number of characters, words, and sentences in a document. “We reasoned that writers from certain linguistic backgrounds may prefer many short sentences, while other writers may prefer fewer but longer sentences.”
Data: TOEFL11 non-native corpus

\item \textbf{CIC-IPN@INLI2018: Indian Native Language Identification (http://ceur-ws.org/Vol-2266/T2-6.pdf )} : 
Features: POS, punctuation, ‘emotion polarity’, word and char n-grams.
Misspellings are extracted from the training data using the PyEnchant package (https://pypi.org/project/pyenchant/) and build character 4-grams from them.
Data: The training dataset released by the organizers of the shared task consists of Facebook comments in the English language extracted from regional language newspapers. “The corpus is collected from texts from regional news paper pages available in Facebook by considering the hypothesis that the user belongs to a particular region will read the news from respective regional news paper.”
\end{itemize}

\subsection{  Misspellings related}

Taxonomy of Spelling mistake sources - keyboard, phonetics etc  

\begin{itemize}
    \item \textbf{Misspelling Oblivious Word Embeddings} :
    Motivation: “One of the most urgent issues of word embeddings is that they are often unable to deal with malformed words which is a big limitation in the real-world applications”
    Dataset: Created using misspellings found in facebook (which were manually corrected by the users) Publicly released here:  \url{https://bitbucket.org/bedizel/moe/src/master/data/moe_misspellings_train.tsv}
    Intrinsic Evaluation: Word similarity and word analogy.
    Extrinsic evaluation: POS tagging
\end{itemize}

\subsection{Second-language Acquisition}
\label{subsec:L2}

There has been a fair amount of interest in the second-language
acquisition field in spelling errors by second-language learners.
For example Flor et al.~\shortcite{Flor:EtAl:15} present an analysis of L1 and L2 English writers
based on data from the Educational Testing Service's spelling corpus
derived from the written essay sections of the GRE and TOEFL
exams, and study contrasts between L1 and L2 learners. More recently, Flor et al.~\shortcite{Flor:EtAl:19} present a corpus of second-language spelling
errors in English from the essay portion of
TOEFL.\footnote{\url{https://github.com/EducationalTestingService/toefl-spell}} 
Unfortunately this work does not investigate the influence of a
learner's L1, and the TOEFL corpus does not provide information on the
first language of the learner.

However, there have been a number of pieces of work that do
investigate L1 influence. Cook~\shortcite{Cook:97} presents a corpus-based study
comparing spelling errors in English from L1 English speakers and L2
learners of English. While many of the errors are not attributed to
particular native language backgrounds, some errors in Cook's corpus
clearly show L1 influence. For example, for Japanese, not only are
there errors involving the familiar confusion of /l/ and /r/, but
Japanese speakers also showed a tendency to add spurious epenthetic
vowels as in \emph{adovocated} for \emph{advocated}, or
\emph{Engilish} for \emph{English}, reflecting an L1 constraint on
consonant clusters. Cook also cites various earlier work showing
examples of L1 influence, such as Ibrahim~\shortcite{Ibrahim:78}, who notes that
Arabic speakers confuse \written{b} and \written{p} since Standard
Arabic lacks a /p/ in its phonological inventory; and
James et al.\shortcite{James:EtAl:93}, who note that ``almost 40\% of attested
misspellings [of Welsh bilinguals writing English] are attributable to
Welsh L1 pronunciation and spelling rules''.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Besten and Granger~\shortcite{Bestgen:Granger:11} compare Spanish-speaking, French-speaking
and German-speaking L2 learners of English, classifying errors into a
number of categories, and showing that certain kinds of errors are
statistically much more likely to occur with some L1 backgrounds than
others. For example, Spanish speakers were more likely than French or
German speakers to make spelling errors that involved double
consonants---\emph{comunity} for \emph{community}. However, it is not
clear to what extent the errors can be attributed to the L1 phonology
as opposed to L1 spelling: Spanish lacks phonological geminates (as
does English), but also lacks orthographic double consonants---e.g.,
\emph{community} is \emph{comunidad} in Spanish.

Sari~\shortcite{Sari:15} looks at errors in English spelling among Indonesian
speaking learners and notes trends such as that Bahasa Indonesia does
not distinguish /s/ and /{\NotoSans ʃ}/, so that \written{sh} is often
misspelled as \written{s}; and for similar reasons \written{ch} is often
misspelled as \written{c}.

Choi and Ryu~\shortcite{Choi:Ryu:17} compare English-speaking learners of Korean, with
\emph{heritage} learners---i.e. children of Korean-speaking parents
who grow up speaking Korean at home, but who learn English in school
and only learn written Korean later in life. Seemingly paradoxically,
heritage learners actually committed \emph{more} spelling errors than
L2 learners. Choi and Ryu attribute this to the fact that the heritage
learners are very familiar with the phonology of Korean, and base
their spelling on the pronunciation, which is often a misleading
guide. Korean spelling is morphophonological, in that it often
reflects morphology or even etymology, and while it is reasonably easy
to predict the pronunciation of a Korean word given its spelling, it
is not always easy to go the other way.  For example, in
{\hangul 괜찮아요} (\emph{kw{\ae}nchan\underline{h}ayo}) `okay', the underlined \written{h} is not pronounced; hence heritage learners may misspell it as 
{\hangul 괜찬아요} (\emph{kw{\ae}nchanayo}).

Kusuran~\shortcite{Kusuran:16} studies spelling errors in Swedish-speaking students
learning English. Some mistakes, such as consonant-doubling can be
attributed to the influence of Swedish spelling conventions: thus
\emph{up} might be misspelled as \emph{upp} due to the latter spelling
being used for the Swedish cognate preposition.

Ogneva~\shortcite{Ogneva:18} studies spelling errors in Spanish-speaking
second-language learners of Russian. She notes a number of types of
error that clearly relate to the influence of native Spanish phonology
on the perception of Russian. For example, palatalized consonants are
frequently represented in Russian orthography in the following vowel,
so that a consonant followed by {\NotoSans е} (\written{e}) is
usually pronounced as a palatal consonant. To Spanish speakers this
sounds like a glide followed by a vowel, and thus Ogneva finds
misspellings such as {\NotoSans интериесный} (\emph{interiesnyj}) in
place of correct {\NotoSans интересный} (\emph{interesnyj})
`interesting'. Similar to Spanish speakers learning in English noted
above in Besten and Granger's~\shortcite{Bestgen:Granger:11} work, Spanish speakers learning
Russian also tend to replace orthographic double consonants (which are
phonologically non-geminate in Russian), with single consonants:
{\NotoSans Руская} (\emph{ruskaja}) for {\NotoSans Русская} (\emph{russkaja})
`Russian'.  One of the most frequent letter substitution errors
involves {\NotoSans б} (\emph{b}) versus {\NotoSans в} (\emph{v}). Spanish uses
both \written{b} and \written{v} in its orthography, but there is no
phonological distinction between the two, which helps explain why
Spanish speakers have difficulty making the distinction in spelling
Russian words.

Finally, Motohashi and Ishizawa\shortcite{Motohashi:Ishizawa:20} study spelling errors in
Japanese hiragana by native English speakers learning Japanese. Errors
that seem to be attributable to phonological distinctions missing in
English are spelling errors involving confusing long and short vowels,
and similarly geminate and non-geminate consonants.

 \subsection{Creoles and Pidgins}

==> old_related_l2_work.tex <==
\subsection{Second-language Acquisition}
\label{subsec:L2}

There has been a fair amount of interest in the second-language
acquisition field in spelling errors by second-language learners.
For example Flor et al.~\shortcite{Flor:EtAl:15} present an analysis of L1 and L2 English writers
based on data from the Educational Testing Service's spelling corpus
derived from the written essay sections of the GRE and TOEFL
exams, and study contrasts between L1 and L2 learners. More recently, Flor et al.~\shortcite{Flor:EtAl:19} present a corpus of second-language spelling
errors in English from the essay portion of
TOEFL.\footnote{\url{https://github.com/EducationalTestingService/toefl-spell}} 
Unfortunately this work does not investigate the influence of a
learner's L1, and the TOEFL corpus does not provide information on the
first language of the learner.

However, there have been a number of pieces of work that do
investigate L1 influence. Cook~\shortcite{Cook:97} presents a corpus-based study
comparing spelling errors in English from L1 English speakers and L2
learners of English. While many of the errors are not attributed to
particular native language backgrounds, some errors in Cook's corpus
clearly show L1 influence. For example, for Japanese, not only are
there errors involving the familiar confusion of /l/ and /r/, but
Japanese speakers also showed a tendency to add spurious epenthetic
vowels as in \emph{adovocated} for \emph{advocated}, or
\emph{Engilish} for \emph{English}, reflecting an L1 constraint on
consonant clusters. Cook also cites various earlier work showing
examples of L1 influence, such as Ibrahim~\shortcite{Ibrahim:78}, who notes that
Arabic speakers confuse \written{b} and \written{p} since Standard
Arabic lacks a /p/ in its phonological inventory; and
James et al.\shortcite{James:EtAl:93}, who note that ``almost 40\% of attested
misspellings [of Welsh bilinguals writing English] are attributable to
Welsh L1 pronunciation and spelling rules''.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Besten and Granger~\shortcite{Bestgen:Granger:11} compare Spanish-speaking, French-speaking
and German-speaking L2 learners of English, classifying errors into a
number of categories, and showing that certain kinds of errors are
statistically much more likely to occur with some L1 backgrounds than
others. For example, Spanish speakers were more likely than French or
German speakers to make spelling errors that involved double
consonants---\emph{comunity} for \emph{community}. However, it is not
clear to what extent the errors can be attributed to the L1 phonology
as opposed to L1 spelling: Spanish lacks phonological geminates (as
does English), but also lacks orthographic double consonants---e.g.,
\emph{community} is \emph{comunidad} in Spanish.

Sari~\shortcite{Sari:15} looks at errors in English spelling among Indonesian
speaking learners and notes trends such as that Bahasa Indonesia does
not distinguish /s/ and /{\NotoSans ʃ}/, so that \written{sh} is often
misspelled as \written{s}; and for similar reasons \written{ch} is often
misspelled as \written{c}.

Choi and Ryu~\shortcite{Choi:Ryu:17} compare English-speaking learners of Korean, with
\emph{heritage} learners---i.e. children of Korean-speaking parents
who grow up speaking Korean at home, but who learn English in school
and only learn written Korean later in life. Seemingly paradoxically,
heritage learners actually committed \emph{more} spelling errors than
L2 learners. Choi and Ryu attribute this to the fact that the heritage
learners are very familiar with the phonology of Korean, and base
their spelling on the pronunciation, which is often a misleading
guide. Korean spelling is morphophonological, in that it often
reflects morphology or even etymology, and while it is reasonably easy
to predict the pronunciation of a Korean word given its spelling, it
is not always easy to go the other way.  For example, in
{\hangul 괜찮아요} (\emph{kw{\ae}nchan\underline{h}ayo}) `okay', the underlined \written{h} is not pronounced; hence heritage learners may misspell it as 
{\hangul 괜찬아요} (\emph{kw{\ae}nchanayo}).

Kusuran~\shortcite{Kusuran:16} studies spelling errors in Swedish-speaking students
learning English. Some mistakes, such as consonant-doubling can be
attributed to the influence of Swedish spelling conventions: thus
\emph{up} might be misspelled as \emph{upp} due to the latter spelling
being used for the Swedish cognate preposition.

Ogneva~\shortcite{Ogneva:18} studies spelling errors in Spanish-speaking
second-language learners of Russian. She notes a number of types of
error that clearly relate to the influence of native Spanish phonology
on the perception of Russian. For example, palatalized consonants are
frequently represented in Russian orthography in the following vowel,
so that a consonant followed by {\NotoSans е} (\written{e}) is
usually pronounced as a palatal consonant. To Spanish speakers this
sounds like a glide followed by a vowel, and thus Ogneva finds
misspellings such as {\NotoSans интериесный} (\emph{interiesnyj}) in
place of correct {\NotoSans интересный} (\emph{interesnyj})
`interesting'. Similar to Spanish speakers learning in English noted
above in Besten and Granger's~\shortcite{Bestgen:Granger:11} work, Spanish speakers learning
Russian also tend to replace orthographic double consonants (which are
phonologically non-geminate in Russian), with single consonants:
{\NotoSans Руская} (\emph{ruskaja}) for {\NotoSans Русская} (\emph{russkaja})
`Russian'.  One of the most frequent letter substitution errors
involves {\NotoSans б} (\emph{b}) versus {\NotoSans в} (\emph{v}). Spanish uses
both \written{b} and \written{v} in its orthography, but there is no
phonological distinction between the two, which helps explain why
Spanish speakers have difficulty making the distinction in spelling
Russian words.

Finally, Motohashi and Ishizawa\shortcite{Motohashi:Ishizawa:20} study spelling errors in
Japanese hiragana by native English speakers learning Japanese. Errors
that seem to be attributable to phonological distinctions missing in
English are spelling errors involving confusing long and short vowels,
and similarly geminate and non-geminate consonants.



==> second_language_acquisition.tex <==

%% TODO(rws): Update this section with a shorter version
\subsection{Second-language Acquisition}
\label{subsec:L2}

There has been a fair amount of interest in the second-language
acquisition field on the influence of native language (L1) on second-language spelling. 
Cook~\shortcite{Cook:97} presents a corpus-based study
comparing spelling errors in English from native speakers and second-language
learners, where some of the errors 
clearly show L1 influence. For example, Japanese speakers showed 
the expected \emph{l-r} confusion,  but there was also a tendency to add spurious epenthetic
vowels as in 
\emph{Eng\textbf{i}lish} for \emph{English}, reflecting an L1 constraint on
consonant clusters. Cook also cites earlier work showing
examples of L1 influence, such as Ibrahim~\shortcite{Ibrahim:78}, 
who notes that Arabic speakers confuse \emph{b} and \emph{p} since Standard
Arabic lacks /p/.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Besten and Granger~\shortcite{Bestgen:Granger:11} compare Spanish-, French-
and German-speaking learners of English, showing that certain kinds of errors are
statistically much more likely to occur with some L1 backgrounds than
others. For example, Spanish speakers were more likely than French or
German speakers to make spelling errors that involved double
consonants---\emph{comunity} for \emph{community}.

Sari~\shortcite{Sari:15} looks at errors in English spelling among Indonesian-speaking learners. For example
Indonesian does
not distinguish /s/ and /\v{s}/, and thus English \emph{sh} is often
misspelled as \emph{s}.

Ogneva~\shortcite{Ogneva:18} studies spelling errors in Spanish-speaking
second-language learners of Russian. She notes a number of errors due to the influence of Spanish phonology
on the perception of Russian. For example, palatalized consonants are
frequently represented in Russian orthography in the following vowel.
To Spanish speakers these
sound like a glide followed by a vowel. Thus Ogneva finds
misspellings such as \emph{inter\textbf{i}esnyj}\footnote{Here we transliterate the Cyrillic originals.}
for \emph{interesnyj}
`interesting'.
One of the most frequent letter substitution errors
involves \emph{b} versus \emph{v}. Spanish uses
both \emph{b} and \emph{v} in its orthography, but they are
phonologically identical, so
Spanish speakers have difficulty making the distinction in spelling
Russian words.

Finally, Motohashi and Ishizawa~\shortcite{Motohashi:Ishizawa:20} study spelling errors in
\emph{hiragana} by English-speaking  learners of Japanese. Spelling errors
apparently attributable to phonological distinctions missing in
English include confusing long and short vowels,
and geminate and non-geminate consonants.


